What's the Difference Between Professional Human and Machine Translation? A Blind Multi-language Study on Domain-specific MT

Machine translation (MT) has been shown to produce a number of errors that require human post-editing, but the extent to which professional human translation (HT) contains such errors has not yet been compared to MT. We compile pre-translated documents in which MT and HT are interleaved, and ask professional translators to flag errors and post-edit these documents in a blind evaluation. We find that the post-editing effort for MT segments is only higher in two out of three language pairs, and that the number of segments with wrong terminology, omissions, and typographical problems is similar in HT.

==> EAMT Proceedings/figures/plots.en.tex <==
\begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[height=5.5cm]{plots/EN-ErrTerminology.pdf}
    \caption{Terminology,\\$p=0.192$}
    \label{fig:PlotsENTerminology}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/EN-ErrOmission.pdf}
    \caption{Omission,\\$p=0.214$}
    \label{fig:PlotsENOmission}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/EN-ErrTypography.pdf}
    \caption{Typography,\\$p=1.000$}
    \label{fig:PlotsENTypography}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/EN-EditMin1.pdf}
    \caption{MED >0,\\$p\leq.05$}
    \label{fig:PlotsENEditMin1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/EN-EditMin6.pdf}
    \caption{MED >5,\\$p=0.255$}
    \label{fig:PlotsENEditMin6}
\end{subfigure}

==> EAMT Proceedings/figures/plots.fr.tex <==
\begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[height=5.5cm]{plots/FR-ErrTerminology.pdf}
    \caption{Terminology,\\$p=0.144$}
    \label{fig:PlotsFRTerminology}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/FR-ErrOmission.pdf}
    \caption{Omission,\\$p=0.693$}
    \label{fig:PlotsFROmission}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/FR-ErrTypography.pdf}
    \caption{Typography,\\$p=0.504$}
    \label{fig:PlotsFRTypography}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/FR-EditMin1.pdf}
    \caption{MED >0,\\$p\leq.05$}
    \label{fig:PlotsFREditMin1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/FR-EditMin6.pdf}
    \caption{MED >5,\\$p\leq.05$}
    \label{fig:PlotsFREditMin6}
\end{subfigure}

==> EAMT Proceedings/figures/plots.it.tex <==
\begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[height=5.5cm]{plots/IT-ErrTerminology.pdf}
    \caption{Terminology,\\$p=1.000$}
    \label{fig:PlotsITTerminology}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/IT-ErrOmission.pdf}
    \caption{Omission,\\$p=0.213$}
    \label{fig:PlotsITOmission}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/IT-ErrTypography.pdf}
    \caption{Typography,\\$p=0.599$}
    \label{fig:PlotsITTypography}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/IT-EditMin1.pdf}
    \caption{MED >0,\\$p=0.110$}
    \label{fig:PlotsITEditMin1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.15\textwidth}
    \centering
    \includegraphics[height=5.5cm,trim={1.8cm 0 0 0},clip]{plots/IT-EditMin6.pdf}
    \caption{MED >5,\\$p=0.674$}
    \label{fig:PlotsITEditMin6}
\end{subfigure}

==> EAMT Proceedings/tables/data.tex <==
\begin{tabular}{lrrr} \toprule
              & \multicolumn{1}{l}{DE--EN} & \multicolumn{1}{l}{DE--FR} & \multicolumn{1}{l}{DE--IT} \\ \midrule
\multicolumn{1}{l}{\textbf{Segments}} \\
~~~ID            & 527,526                    & 1,177,704                  & 905,302                    \\
~~~OOD           & 20,000,000                 & 7,760,035                  & 6,925,296                  \\
~~~Ratio~~~      & 10:1                       & 6:1                        & 7:1                        \\[0.5em]
\textbf{Terms}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       \\
~~~Train         & 10,332                     & 11,551                     & 10,537                     \\
~~~Test          & 3,256                      & 4,915                      & 4,817                      \\ \bottomrule
\end{tabular}

==> EAMT Proceedings/tables/error.definitions.tex <==
\begin{tabularx}{\columnwidth}{lX}
\toprule
\textbf{Error Type} & \textbf{Definition (MQM)}                                                                                                             \\ \midrule
Terminology         & A term (domain-specific word) is translated with a term other than the one expected for the domain or otherwise specified.            \\
Omission            & Content is missing from the translation that is present in the source.                                                                \\
Typography          & Issues related to the mechanical presentation of text. This category should be used for any typographical errors other than spelling. \\ \bottomrule
\end{tabularx}

==> EAMT Proceedings/tables/fisher.example.tex <==
\begin{tabular}{lrr}
\toprule
            & \multicolumn{1}{l}{HT} & \multicolumn{1}{l}{MT} \\ \midrule
Omission    & 14                     & 12                     \\
No Omission & 223                    & 226                    \\ \midrule
Total       & 237                    & 238                    \\ \bottomrule
\end{tabular}

==> EAMT Proceedings/tables/materials.example.tex <==
\begin{tabularx}{\textwidth}{lXXl} \toprule
\textbf{ID} & \textbf{Source (DE)}                  & \textbf{Target (EN)}          & \textbf{Origin} \\ \midrule
1 & Dieses Arbeitspapier beschränkt sich auf die notwendigen Funktionalitäten für die Bestandsführung.&	This \textbf{work paper} is limited to the necessary functions for portfolio management. & MT \\
\midrule
2 &Das Kapitel zur Benutzerverwaltung befindet sich noch in Erstellung.&	The user administration chapter is still being prepared. & MT \\
\midrule
3 & Voraussetzungen &	Requirements\textbf{:} & HT \\
 \midrule
4 & Die in der Lohnbuchhaltung erfassten Personen müssen voll arbeitsfähig sein.&	The persons entered in payroll accounting must be fully capable of working. & HT \\
 \midrule
5 & Es werden weiters ausschliesslich Personen mit Jahreslohn adressiert und keine Personen, welche auf Stundenlohnbasis arbeiten.&	Furthermore, only persons receiving an annual salary are addressed and not persons working on an hourly wage basis. & HT \\
 \midrule
6 &Für die später beschriebenen Mutationen \textbf{inkl. Eintritt / Austritt} wird von der Web API eine Korrelations ID zurückgegeben.&	A correlation ID is returned by the Web API for the changes described later. & MT \\
 \bottomrule
\end{tabularx}

==> EAMT Proceedings/tables/results.error-analysis.tex <==
\begin{tabular}{rrrrrr} \specialrule{1pt}{0.5em}{0.5em}
\multicolumn{2}{l}{Terminology}                 & \multicolumn{2}{l}{Omission}                    & \multicolumn{2}{l}{Typography}                  \\[0.2em]
\multicolumn{1}{l}{\#} & \multicolumn{1}{l}{\%} & \multicolumn{1}{l}{\#} & \multicolumn{1}{l}{\%} & \multicolumn{1}{l}{\#} & \multicolumn{1}{l}{\%} \\[0.5em] \specialrule{0.5pt}{0pt}{0.5em}
8                      & 5.33                   & 1                      & 0.67                   & 3                      & 2.00                   \\
15                     & 10                     & 5                      & 3.33                   & 4                      & 2.67                   \\[0.5em]
27                     & 11.39                  & 14                     & 5.91                   & 5                      & 2.11                   \\
39                     & 16.39                  & 12                     & 5.04                   & 3                      & 1.26                   \\[0.5em]
18                     & 7.38                   & 4                      & 1.64                   & 8                      & 3.28                   \\
19                     & 7.66                   & 1                      & 0.40                   & 6                      & 2.42                   \\[0.5em] \bottomrule
\end{tabular}

==> EAMT Proceedings/tables/results.post-editing.tex <==
\begin{tabular}{lllrlrrrrrl} \specialrule{1pt}{0.5em}{0.5em}
Data                &                    &          & \multicolumn{1}{l}{}   &  & \multicolumn{6}{l}{Post-editing}                                                                                                      \\[0.5em]
Language            & Raters             & Segments & \multicolumn{1}{l}{}   &  & \multicolumn{5}{l}{Minimum Edit Distance}                                                                                      & HTER \\[0.2em]
                    &                    & Origin   & \multicolumn{1}{l}{\#} &  & \multicolumn{1}{l}{min} & \multicolumn{1}{l}{max} & \multicolumn{1}{l}{avg} & \multicolumn{1}{l}{med} & \multicolumn{1}{l}{sd} &      \\[0.5em] \specialrule{0.5pt}{0pt}{0.5em}
\multirow{2}{*}{EN} & \multirow{2}{*}{2} & HT       & 150                    &  & 0                       & 85                      & 1.56                    & 0                       & 7.85                   & 2.22 \\
                    &                    & MT       & 150                    &  & 0                       & 43                      & 2.89                    & 0                       & 7.86                   & 4.71 \\[0.5em]
\multirow{2}{*}{FR} & \multirow{2}{*}{4} & HT       & 237                    &  & 0                       & 118                     & 6.89                    & 0                       & 17.41                  & 7.42 \\
                    &                    & MT       & 238                    &  & 0                       & 150                     & 7.83                    & 0                       & 17.43                  & 7.99 \\[0.5em]
\multirow{2}{*}{IT} & \multirow{2}{*}{4} & HT       & 244                    &  & 0                       & 34                      & 2.39                    & 0                       & 6.17                   & 3.67 \\
                    &                    & MT       & 248                    &  & 0                       & 130                     & 2.92                    & 0                       & 13.07                  & 3.81 \\[0.5em] \bottomrule
\end{tabular}

==> EAMT Proceedings/tables/results.tex <==
\begin{tabular}{lrrrrrrrrrrrr} \specialrule{1pt}{0.5em}{0.5em}
                        & \multicolumn{4}{c}{\textbf{DE--EN}}                                                                                             & \multicolumn{4}{c}{\textbf{DE--FR}}                                                                                             & \multicolumn{4}{c}{\textbf{DE--IT}}                                                               \\[0.2em]
                        & \multicolumn{2}{l}{\textbf{HT} (N=150)}                                 & \multicolumn{2}{l}{\textbf{MT} (N=150)}                                 & \multicolumn{2}{l}{\textbf{HT} (N=237)}                                 & \multicolumn{2}{l}{\textbf{MT} (N=238)}                                 & \multicolumn{2}{l}{\textbf{HT} (N=244)}                  & \multicolumn{2}{l}{\textbf{MT} (N=248)}                  \\ [0.5em] \specialrule{0.5pt}{0pt}{0.5em}
\textbf{Error Analysis} &                            &                                   &                            &                                   &                            &                                   &                            &                                   &                          &                      &                          &                      \\
~~~Terminology          & 8                          & \hspace{-3mm}(5.33)                          & 15                         & \hspace{-3mm}(10.00)                         & 27                         & \hspace{-3mm}(11.39)                         & 39                         & \hspace{-3mm}(16.39)                         & 18                       & \hspace{-3mm}(7.38)             & 19                       & \hspace{-3mm}(7.66)             \\
~~~Omission             & 1                          & \hspace{-3mm}(0.67)                          & 5                          & \hspace{-3mm}(3.33)                          & 14                         & \hspace{-3mm}(5.91)                          & 12                         & \hspace{-3mm}(5.04)                          & 4                        & \hspace{-3mm}(1.64)             & 1                        & \hspace{-3mm}(0.40)             \\
~~~Typography           & 3                          & \hspace{-3mm}(2.00)                          & 4                          & \hspace{-3mm}(2.67)                          & 5                          & \hspace{-3mm}(2.11)                          & 3                          & \hspace{-3mm}(1.26)                          & 8                        & \hspace{-3mm}(3.28)             & 6                        & \hspace{-3mm}(2.42)             \\[0.5em]
\multicolumn{13}{l}{\textbf{MED}}                                                                                                                                                                                                                                                                                                                                                               \\
~~~\textgreater 0       & *\,20 & \hspace{-3mm}(13.33) & *\,37 & \hspace{-3mm}(24.67) & *\,67 & \hspace{-3mm}(28.27) & *\,90 & \hspace{-3mm}(37.82) & 65                       & \hspace{-3mm}(26.64)            & 50                       & \hspace{-3mm}(20.16)            \\
~~~\textgreater 5       & 12                         & \hspace{-3mm}(8.00)                          & 19                         & \hspace{-3mm}(12.67)                         & *\,53 & \hspace{-3mm}(22.36) & *\,75 & \hspace{-3mm}(31.51) & 30                       & \hspace{-3mm}(12.30)            & 27                       & \hspace{-3mm}(10.89)            \\[0.5em]
~~~min                  & 0                          &                                   & 0                          &                                   & 0                          &                                   & 0                          &                                   & 0                        &                      & 0                        &                      \\
~~~max                  & 85                         &                                   & 43                         &                                   & 118                        &                                   & 150                        &                                   & 34                       &                      & 130                      &                      \\
~~~avg                  & 1.56                       &                                   & 2.89                       &                                   & 6.89                       &                                   & 7.83                       &                                   & 2.39                     &                      & 2.92                     &                      \\
~~~med                  & 0                          &                                   & 0                          &                                   & 0                          &                                   & 0                          &                                   & 0                        &                      & 0                        &                      \\
~~~sd                   & 7.85                       &                                   & 7.86                       &                                   & 17.41                      &                                   & 17.43                      &                                   & 6.17                     &                      & 13.07                    &                      \\[0.5em]
\textbf{HTER}           &                            &                                   &                            &                                   &                            &                                   &                            &                                   &                          &                      &                          &                      \\
~~~Corpus-level         & \multicolumn{1}{l}{2.22}   & \multicolumn{1}{l}{}              & \multicolumn{1}{l}{4.71}   & \multicolumn{1}{l}{}              & \multicolumn{1}{l}{7.42}   & \multicolumn{1}{l}{}              & \multicolumn{1}{l}{7.99}   & \multicolumn{1}{l}{}              & \multicolumn{1}{l}{3.67} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{3.81} & \multicolumn{1}{l}{} \\ \bottomrule
\end{tabular}

==> tables/results.error-analysis.tex <==
\begin{tabular}{rrrrrr} \specialrule{1pt}{0.5em}{0.5em}
\multicolumn{2}{l}{Terminology}                 & \multicolumn{2}{l}{Omission}                    & \multicolumn{2}{l}{Typography}                  \\[0.2em]
\multicolumn{1}{l}{\#} & \multicolumn{1}{l}{\%} & \multicolumn{1}{l}{\#} & \multicolumn{1}{l}{\%} & \multicolumn{1}{l}{\#} & \multicolumn{1}{l}{\%} \\[0.5em] \specialrule{0.5pt}{0pt}{0.5em}
8                      & 5.33                   & 1                      & 0.67                   & 3                      & 2.00                   \\
15                     & 10                     & 5                      & 3.33                   & 4                      & 2.67                   \\[0.5em]
27                     & 11.39                  & 14                     & 5.91                   & 5                      & 2.11                   \\
39                     & 16.39                  & 12                     & 5.04                   & 3                      & 1.26                   \\[0.5em]
18                     & 7.38                   & 4                      & 1.64                   & 8                      & 3.28                   \\
19                     & 7.66                   & 1                      & 0.40                   & 6                      & 2.42                   \\[0.5em] \bottomrule
\end{tabular}

==> tables/results.post-editing.tex <==
\begin{tabular}{lllrlrrrrrl} \specialrule{1pt}{0.5em}{0.5em}
Data                &                    &          & \multicolumn{1}{l}{}   &  & \multicolumn{6}{l}{Post-editing}                                                                                                      \\[0.5em]
Language            & Raters             & Segments & \multicolumn{1}{l}{}   &  & \multicolumn{5}{l}{Minimum Edit Distance}                                                                                      & HTER \\[0.2em]
                    &                    & Origin   & \multicolumn{1}{l}{\#} &  & \multicolumn{1}{l}{min} & \multicolumn{1}{l}{max} & \multicolumn{1}{l}{avg} & \multicolumn{1}{l}{med} & \multicolumn{1}{l}{sd} &      \\[0.5em] \specialrule{0.5pt}{0pt}{0.5em}
\multirow{2}{*}{EN} & \multirow{2}{*}{2} & HT       & 150                    &  & 0                       & 85                      & 1.56                    & 0                       & 7.85                   & 2.22 \\
                    &                    & MT       & 150                    &  & 0                       & 43                      & 2.89                    & 0                       & 7.86                   & 4.71 \\[0.5em]
\multirow{2}{*}{FR} & \multirow{2}{*}{4} & HT       & 237                    &  & 0                       & 118                     & 6.89                    & 0                       & 17.41                  & 7.42 \\
                    &                    & MT       & 238                    &  & 0                       & 150                     & 7.83                    & 0                       & 17.43                  & 7.99 \\[0.5em]
\multirow{2}{*}{IT} & \multirow{2}{*}{4} & HT       & 244                    &  & 0                       & 34                      & 2.39                    & 0                       & 6.17                   & 3.67 \\
                    &                    & MT       & 248                    &  & 0                       & 130                     & 2.92                    & 0                       & 13.07                  & 3.81 \\[0.5em] \bottomrule
\end{tabular}
